TwIPS: A Large Language Model Powered Texting Application to Simplify Conversational Nuances for Autistic Users

Autistic individuals often experience difficulties in conveying and interpreting emotional tone and non-literal nuances. Many also mask their communication style to avoid being misconstrued by others, spending considerable time and mental effort in the process. To address these challenges in text-based communication, we present TwIPS, a prototype texting application powered by a large language model (LLM), which can assist users with: a) deciphering tone and meaning of incoming messages, b) ensuring the emotional tone of their message is in line with their intent, and c) coming up with alternate phrasing for messages that could be misconstrued and received negatively by others. We leverage an AI-based simulation and a conversational script to evaluate TwIPS with 8 autistic participants in an in-lab setting. Our findings show TwIPS enables a convenient way for participants to seek clarifications, provides a better alternative to tone indicators, and facilitates constructive reflection on writing technique and style. We also examine how autistic users utilize language for self-expression and interpretation in instant messaging, and gather feedback for enhancing our prototype. We conclude with a discussion around balancing user-autonomy with AI-mediation, establishing appropriate trust levels in AI systems, and customization needs if autistic users in the context of AI-assisted communication

==> alt-text.tex <==
%Figure 1
This figure shows a screenshot of the layout of TwIPS, with a conversation in progress. At the top left, there is a picture featuring an avatar with the name "Jimmy" next to it. The conversation in this screenshot begins with a message from a hypothetical participant, saying, "hey! how are you doing?", to which Jimmy replies on the left with, "hey! i'm good, thanks. what's going on?" The next message from the participant on the right is, "do you want to join me on a trip to gloucester this weekend?". Jimmy responds on the left, "gloucester, huh? sounds like a blast! what's the plan, mate?"

At the bottom of the interface, there is a text input field with the placeholder text "type your message here" and three distinct buttons. On the left of the text input field is the preview button and an emoji to toggle the emoji menu, and on the right, there is a send button represented by an arrow icon. The background of the interface is dark, and the chat bubbles are contrasting, with Jimmy's in white and the participants in a darker shade. In this way, the layout of TwIPS mirrored a standard, modern instant messaging application.


%Figure 2a
This figure is a screenshot of a close-up of a single message within TwIPS' layout. The chat bubble is white with black text inside it and is positioned against a dark background. The text reads, "gloucester, huh? sounds like a blast! what's the plan, mate?" There's a small, circular gray symbol in the upper left corner of the message bubble, indicating that this message contains potentially ambiguous language elements. The symbol serves as a marker for received messages that might need the receiver's further attention. This enabled us to subtly highlight messages that could be potentially ambiguous.

%Figure 2b

This image features a close-up of the same text message as in the previous figure. The message bubble is white with black text, and it's set against a dark background. The text inside the message bubble reads: "gloucester, huh? sounds like a blast! what's the plan, mate?" A section of the text, "sounds like a blast!" is underlined, indicating that this phrase has been identified as potentially ambiguous. A mouse cursor appears to the right of the underlined text within the message bubble, indicating that the underlining is a result of hovering the cursor over the message bubble. In this way, hovering the cursor over any message bubble containing the gray circular symbol (indication potential ambiguity) underlines the ambiguous element(s).


%Figure 2c
This figure features a close-up of the same text message as in the previous two figures. The message bubble is white with black text, and it's set against a dark background. The message reads, "gloucester, huh? sounds like a blast! what's the plan, mate?" The phrase "sounds like a blast!" is underlined, and a cursor hovers over the underlined text, showing that the user has clicked on the underline phrase. Below the underlined phrase is a smaller, secondary text bubble within the main text bubble containing an explanatory note which reads: "The phrase 'sounds like a blast!' implies that the trip to Gloucester seems very exciting and fun." The explanatory note's bubble has a lighter background and rounded corners. In this way, users could click on any language element that was underlined and receive an explanation for it.

%Figure 2d:

The second figure features a close-up of the same text message as in the previous three figures. However, this time, the user has clicked on a non-underlined segment of the message bubble. As a result, below the main message is a secondary text bubble, which provides a brief description of the overall tone and meaning of the message. It reads, "Tone: Enthusiastic and Friendly. Meaning: The person is excited about the prospect of going to Gloucester and is asking for more details about the trip." In this way, by clicking anywhere in the message bubble other than the underlined language elements, users could get an overall tone and meaning of any message. 


%Figure 3a:

This image is a close-up screenshot of the message writing box and its surrounding user interface (UI) elements, showing the Preview feature in action. On the left, there's an emoji button for users to toggle the emojis menu, and another button labeled "Preview Button". On the right,there is a green send button with an arrow icon. The central part of the image shows a text input area where a user has typed this message to send: "we can do canoeing and scuba diving. gloucester is known for water sports all over massachusetts!" Below this message, a secondary, lighter text box contains a feedback generated by the Preview feature that reads, "The other user will likely feel excited and enthusiastic about the proposed activities, given the positive tone and invitation to engage in popular local sports." At the far right, there's a cancel or close button with an "x" icon, to hide the text box containing the feedback. In this example, the message and
preview's feedback were fairly positive, hence Suggest was not triggered and an alternative message was not produced.

%Figure 3b:

This image is a close-up screenshot of the message writing box and its surrounding user interface (UI) elements, showing the Preview and Suggest feature, both, in action. On the left of the message writing box, there's an emoji button for users to toggle the emojis menu, and another button next to it labeled "Preview Button". Users can click on this button to toggle the Preview feature. On the right, there is a green send button with an arrow icon. The central part of the image shows the message writing box where a user has typed the following message to send: "we can do canoeing and scuba diving, but it is a little expensive. you think you can afford it?" Below this message writing box, a secondary, lighter text box contains the feedback generated by the Preview feature corresponding to that message, which reads: "The other user might feel slightly uncomfortable due to the directness regarding affordability. Instead, you might want to say: "We could arrange for canoeing and scuba diving, though it's a bit on the pricey side. Do you think it could work for your budget?"". Within the secondary text box to the right, there is a green button labeled "Copy Suggestion" for easy use of the alternative message suggested, and a cancel or close button next to it with an "x" icon, that users can click to hide the secondary text box.

%Figure 4

This figures shows the setup for phase 1 of the user-study. 2 computer monitors side by side are shown in the figure; the left screen displays the TwIPS' interface with a conversation showing alternating messages from 'Ben' and the study 'User', and a text input area labeled "write message here…" with a send button next to it. The right screen displays the text "Model Response," indicating where the model-generated response appeared. An arrow points to the text input area on the left screen from the model response on the right screen, showing that participants could see and copy the model response from the right screen to the message writing box. The model response on the right screen was updated each time Ben sent a new message.


%Figure 5 Summary

This figure shows the prompt template and flow for clicking on the Preview button. When the user clicks on the preview button, an LLM call is made to determine the bluntness of the user's message out of 10. If the bluntness is greater than 3, another LLM call is made to generate a preview of the user's likely reaction, as well as a less blunt, alternate suggestion. If it is less than 3, only the preview is generated in a separate call.


%Figure 6 Summary

This figure shows the prompt template and flow for clicking on the Send button. When the user clicks on the preview button, an LLM call is made to determine the bluntness of the user's message out of 10. If the bluntness is greater than 3, another LLM call is made to generate a preview of the user's likely reaction, as well as a less blunt, alternate suggestion. If not, no further processing happens. At the same time, a call to the generate the overall tone and meaning of the message and another call to identify any ambiguous language element is made.

%Figure 7 Summary

This figure shows the prompt template and flow for clicking on an underlined language element in a message. Upon clicking, an LLM call to explain that language element is made.


%Table 1 Summary

This table shows information about participants. P1, P2, P3, and P8 had received a formal autism diagnosis while the rest 4 participants self-identified as autistic. P1 was aged 25-34, P4 was aged 35-44 and all other participants were aged 18-24. P1, P2, P4 and P8 identified as female. P3 and P6 identified as non-binary/third gender, and P5 and P6 identified as male. All participants reported their texting usage was "very frequent".

%Table 2

This table summarizes the qualitative feedback and suggestions for improvements provided by participants for each of 3 features in TwIPS.

==> previous-stuff/findingsPrev.tex <==
\section{Findings}

\subsection{Communication Styles}


\subsection{Survey results}
The results from our 7-point Likert scale survey revealed that all six participants favored continued use of the three main features in their everyday chatting apps. {\sc{Interpret}} received the highest rating (Average 6.3, SD = 0.5), closely followed by {\sc{Preview}} (Average = 6.3, SD = 0.47), and {\sc{Suggest}} (Average = 5.33, SD = 1.11). The participants did not perceive the app's ability to generate and suggest alternative messages as a threat to user autonomy (Average = 1.66, SD = 0.47). However, participants felt that {\sc{Preview's}} ability to prevent a message from being sent could have some negative impact on user autonomy (Average = 3, SD = 1.41). There exists a need for more personalized message suggestions, as participants did not strongly feel that the suggestions were representative of their personal communication style (Average = 2.83, SD = 1.46). Overall, there was strong consensus that our prototype enhanced participants' text messaging experience (Average = 6, SD = 0.577). In the following sub-sections, we delve into the qualitative responses from Participant 1.

\subsection{Written Communication Style and Preferences}

P1 emphasized on the use of punctuation in text messages. They associated imperfect punctuation or spelling with an amicable or colloquial tone, and linked precise punctuation to seriousness or more intense emotions like bluntness or annoyance. In addition, P1 mentioned that they often provide explanations for their choice of punctuation: 

\begin{quotation}{\it ``I usually include a lot of context... if I use a specific punctuation mark, I'll explain its purpose. "}\end{quotation}

By `context,' P1 was referring to the addition of tone indicators such as /sarcastic or /excited at the end of a message to explicitly communicate the sender's tone. Although P1 found tone indicators to be useful, they pointed out that they refrain from joking with people who barely know them, because they have been misinterpreted by a lot of people in the past. P1 emphasized the importance of maintaining a balance in textual conversation, particularly when communicating with neurotypical individuals. They illustrated this with an example from their interaction with Ben. \begin{quotation}{\it ``When Ben asked [if I liked] horror films, I realized that saying 'no' would pass the responsibility back to Ben to propose something else. Instead, I thought it's better to also suggest an alternative, like a romantic comedy."}\end{quotation} They claimed that maintaining balance is crucial for mutual engagement but not instinctive for many autistic people they have encountered, who often tend to respond only to the question asked without contributing further to the conversation's continuity. According to them, this tendency can inadvertently convey a lack of interest in engaging to neurotypical people. To tackle this challenge, P1 expressed that, \begin{quotation}{\it "...I constantly try to monitor and balance who's asking the questions. If I've been asked several questions, I make an effort to reciprocate."}\end{quotation}

P1 believed that gender differences can impact others expectations of how one would communicate with them. Being a women, she felt that there was an expectation to soften her language, often necessitating the use of exclamation points or striving to appear excessively kind. This expectation sometimes altered the true intent of her messages, a phenomenon they've frequently encountered. Highlighting the challenge of balancing genuity with societal expectations in text-based conversations, she stated: \begin{quotation} \it ``It's really easy for me to feel like it [masking] is changing what I mean."\end{quotation}





\subsection{Feedback on our Prototype}

P1 found {\sc{Interpret}} useful, though before using our application, they expressed concerns about its accuracy. After the study's completion, they felt it could effectively grasp the context and gist of the message. They believed that the overall meaning provided by {\sc{Interpret}} could be beneficial in a variety of scenarios where undertones and nuances were unclear, such as a confrontation or a message with vague humor. One such instance was where Ben joked with P1, leading to confusion about his intent:

\begin{quotation}
{\it "...I was like, what the hell?  [{\sc Interpret}] helped me understand it was meant to be a joke, telling me that Ben was just being playful."}\end{quotation}


For P1, the tone of a message held situational relevance. For example, tone might be less crucial in planning enjoyable activities compared to more serious conversations. In instances where tone was unclear, they mentioned that they personally ask for clarification directly from the sender, yet they recognized that the application's ability to provide the overall tone of the message could be useful for those less inclined to ask directly. P1 also expressed that constantly explaining one's tone in a message could be tiring, and this feature could serve as an effective alternative:

\begin{quotation}
{\it "It can sometimes be exhausting [for neurotypical individuals] to have to constantly explain what they say to people. [{\sc {Interpret}}] would allow people like me to perhaps investigate the tone without having to have that person write out a whole extra thing. "}\end{quotation}


In phase 1, P1 was able to detect all of the scripted blunt messages. When {\sc{Preview}} was triggered by one of the blunt messages in phase 1, P1 readily agreed with the feedback provided:

\begin{quotation}
    \it ``See! That is exactly what I was saying. I agree with this. I think that [the preview] is a very clear sentence."
\end{quotation}


While sharing her personal experiences, P1 expressed the need to sound non-confrontational, especially in emails. This struggle was evident in situations where their straightforwardness was often misinterpreted as criticism. P1 mentioned this extends beyond emails to text messages, where they frequently rely on their friends for feedback before sending a message. According to them, {\sc{Preview}} would be useful as the current method: \begin{quotation} \it``...requires the help of a community where I have to send screenshots to my friends and be like `Does this sound okay to you?' and rewrite it until it doesn't sound mean." \end{quotation} 

After phase 2, P1 was happy to see that they could now toggle {\sc{Preview}} manually. While they acknowledged the benefits of manual control, they emphasized the importance of {\sc{Preview}} maintaining a proactive approach:

\begin{quotation}{\it "Many autistic people often don't realize when we're being too blunt or saying something off until it's pointed out. So, using the preview button might require a level of self-awareness that we often lack."}\end{quotation} 

P1 saw immense benefit of {\sc{Preview}} for autistic men, pointing out that many autistic women, including themselves, are often diagnosed with ASD later in life and have developed effective masking strategies by that time. Contrarily, P1 highlighted the lack of self-reflection among autistic men they know: \begin{quotation}
   \it ``This could provide really useful self-reflection for a lot of autistic men who, I think, need it. I don't know a single autistic man who wouldn't benefit from this." \end{quotation} They noted that in their discussions about the nuances of communication with autistic men, the typical response is an unfamiliarity with these aspects of communication.

   





\subsection{Improvements and Suggestions}

As P1 emphasized the significance of ensuring balanced participation from both parties in a conversation, they wondered if {\sc{Preview}} could proactively nudge the user to contribute to the conversation's continuity as well. This would be beneficial in situations where one party relies heavily on the other to initiate questions and propose ideas: \begin{quotation}{\it "...the app could prompt me to think about how I can continue the conversation...This way, the conversation feels more like a collaborative effort rather than a series of questions and answers."}\end{quotation}

The process of continuous revision to strike the right tone, while still conveying their original intent, was described as exhausting and one of their biggest communication challenges. At the same time, P1 felt it was important to balance  avoiding bluntness and maintaining authenticity in expressing one's feelings. To address this, they recommended a disclaimer or notification that reminds users to preserve their emotional integrity, ensuring that users do not feel compelled to prioritize the comfort of others over their own honest expression.


P1 found {\sc{Interpret}} to be quite accurate but expressed concerns about the sender's inability to see how their message is interpreted by the receiver. They argued that understanding the receiver's perspective would enable the sender to clarify their message when necessary. Furthermore, P1 suggested adding a toggle feature to {\sc{Preview}}, allowing users to disable its proactive behavior, especially in instances where it is overly sensitive or triggers too often.

\begin{quotation}{\it}\end{quotation}

==> previous-stuff/introduction-pre.tex <==

\section{Introduction}


% Autism Spectrum Disorder (ASD) is one of the most common neuro-developmental disorder, currently observed at a prevalence rate of approximately 1 in 36 among 8-year-old children in the United States, as per the latest data from the Centers for Disease Control and Prevention (CDC) \cite{cdc-prevalence}. Autistic individuals often experience challenges in communication and social interaction, display restricted interests and repetitive behaviors, and exhibit symptoms that can impair their functional capabilities in educational, occupational, and various other, similar contexts \cite{dsm5}. ASD is referred to as a "spectrum" disorder due to the broad range of symptoms and the varying degrees of severity experienced by autistic individuals. From a medical standpoint, this definition is good.

% \advisor{Intro reads well. Good job!
% Two possible things to consider: i) perhaps give a little more importance to generative AI, recent advances and its applications, and how your problem is challenging but generative AI gives us a tool to potentially attack it. ii) the interfaces seem too involved for the intro. May consider just giving a concrete textual example in the intro and leaving the screenshots for a later section? Alternatively, find a way to get the user to only focus on where the action is; otherwise it's too much for the intro.   }

Autism Spectrum Disorder (ASD) is viewed from a medical lens as a complex neuro-developmental disorder. It is characterized by challenges in verbal and nonverbal communication, difficulties in social interactions, repetitive behaviors, and/or sensory sensitivities \cite{dsm5} \cite{grossi-patterns-of}. ASD is one of the most common neuro-developmental disorders in the United States, currently observed at a prevalence rate of approximately 1 in 36 among 8-year-old children \cite{cdc-prevalence}. The term `spectrum' in ASD reflects the broad range of symptoms and the varying degrees of severity experienced by autistic individuals. Accessibility researchers in Human-Computer Interaction (HCI) have extensively utilized technology to enhance autism diagnosis methods \cite{debelen-eyexplain-autism}\cite{arshad-east-early}, therapeutic interventions \cite{gesture-therapy}\cite{jeong-lexical-representation}, social support tools \cite{tartaro-virtual-peer} \cite{washington-a-wearable}, and the overall quality of life \cite{anxiety-autism} \cite{kim-routineaid-externalizing} of autistic individuals. In addition, they have also advocated for the redesign of existing, mainstream applications, such as social media platforms, to better meet the usability needs of autistic users \cite{grynszpan-human-computer}\cite{rapp-interactive-urban}\cite{kender-autism-design}.

%In addition, they have also advocated for the redesign of popular, existing systems like mainstream social media platforms to better accommodate the usability needs of autistic users \cite{grynszpan-human-computer}\cite{rapp-interactive-urban}.

%Accessibility researchers in Human-Computer Interaction (HCI) have not only utilized technology for developing new systems to enhance autism diagnosis methods \cite{debelen-eyexplain-autism}\cite{arshad-east-early}, therapeutic interventions \cite{gesture-therapy}\cite{jeong-lexical-representation}, social support tools \cite{tartaro-virtual-peer} \cite{washington-a-wearable}, and the overall quality of life \cite{anxiety-autism} \cite{kim-routineaid-externalizing} of autistic individuals, but also advocated for the redesign of popular, existing systems, like mainstream social media platforms, to better accommodate the usability needs of autistic users \cite{grynszpan-human-computer} \cite{rapp-interactive-urban}. 

Many autistic individuals find it challenging to process non-verbal cues, such as facial expressions and body language, in face-to-face (FTF) interactions. Expressing and understanding variations in vocal pitch, tone, and loudness can add more layers of complexity to communication, making FTF interactions strenuous and overwhelming. Prior work in disabilities and linguistics underscores a preference for written communication among autistic individuals, highlighting a tendency towards email and text messaging over FTF interactions \cite{howard-anything-but}. This preference is attributed to the greater control and sensory ease provided by written communication as compared to FTF interactions \cite{nicolaidis-respect-healthcare}. %Given the popularity of text-based communication among autistic individuals, it becomes crucial to evaluate whether the design of existing platforms that support text-based communication cater to their needs. 
Through focus groups and in-depth qualitative interviews conducted with autistic users in prior work, researchers have identified that autistic users face challenges in conveying and interpreting emotions, tone and non-literal language, concluding that standard chat features like GIFs and emojis do not address these challenges adequately \cite{barros-my-perfect} \cite{page-perceiving-affordances}. Informed by ideation with autistic users and their specific communication needs detailed in these studies, we introduce \textit{TwIPS}, a prototype texting interface leveraging recent advances in generative AI \cite{gpt4-openai-and}, which enable it to grasp nuanced and implicit elements like intent and context from text. Based on its understanding of these elements, it can dynamically generate feedback for users that is tailored to the specificities of each conversation. TwIPS comprises of three features (described in detail in \secref{sec:prototype-overview}) not found in traditional chatting applications, all of which are powered by GPT4\cite{gpt4-openai-and}:
\begin{enumerate}
    \item {\sc Interpret}: describes the overall tone and meaning of incoming messages, as well as individually identifies and explains ambiguous language elements, such as figurative language, sarcasm, and emojis.
    \item {\sc Preview}: allows users to preview recipients' likely emotional reaction to their message, helping them verify the emotional tone of their message comes across as intended to the recipient and make adjustments if needed.
    \item {\sc Suggest}: complements {\sc Preview} by suggesting a differently phrased alternate message while ensuring the intent of the original message remains preserved but the alternative has a softer tone.
\end{enumerate}


Through an in-lab evaluation with 8 autistic participants recruited from a university setting, ranging in age from 18 to 44, we gathered detailed qualitative feedback and survey responses on their a) perceptions of autonomy, accessibility and usefulness of the TwIPS prototype, and b) use of language for self-expression and interpretation in instant messaging. Our 7-point Likert scale post-study survey revealed that 7 out of 8 participants favored continued use of the three features in their everyday chatting apps, with {\sc{Interpret}} receiving the highest rating (avg. 6.25, s.d = 1.03), followed by {\sc{Preview}} (avg. = 5.88, s.d = 1.64), and {\sc{Suggest}} (avg = 5.13, s.d = 1.72) \footnote{For each feature, participants were asked to express their level of disagreement (1) or agreement (7) with the statement "I would like to continue using the \textit{X} feature in my everyday chatting app", where \textsc{X} was the name of the feature.}. Qualitative data showed that TwIPS enabled a convenient way for users to seek clarifications, provided a better alternative to tone indicators, and facilitated constructive reflection on writing technique. Suggestions for improving it centered on offering greater personalization and implementing measures to prevent users from over-relying on it. While our participants demonstrated a strong desire to actively contribute to conversations rather than allowing them to be one-sided, they indicated achieving this balance was challenging in text-based communication. We believe our work has implications for both accessibility researchers and the broader human-computer interaction (HCI) community around balancing user-autonomy alongside AI-mediation, appropriating users’ trust levels in AI systems, and identifying autistic users’ needs in the context of AI-assisted communication. We conclude by advocating for the need and opportunity to design interventions that distribute accountability and responsibility for reducing communication breakdowns
equitably across all users, instead of placing it solely on autistic users. 

%Our work has implications for future efforts aimed at utilizing generative AI to enhance digital communication modes for autistic users, as well is in other, broader contexts involving human-AI collaboration.

%We believe these considerations have significant implications for the design and deployment of generative AI systems tailored to the specific needs of the autistic community as well as for their broader application.

While we focus on evaluating TwIPS with an autistic audience in this study, we recognize social interactions as an inherently collaborative process. Drawing inspiration from the double empathy problem \cite{damian-on-the}, we believe communication challenges between neurodivergent and neurotypical individuals arise primarily due to differing expectations and communication styles, so neurodiversity should not only be acknowledged but celebrated. Hence, we advocate for deploying versions of our prototype across both autistic and neurotypical users of chatting applications, ensuring that the responsibility to enhance communication is shared more evenly among all users.
%Proponents of neurodiversity argue any challenges encountered by autistic individuals reflect different ways of being that are all part of normal human experiences. 
%They emphasize on the unique strengths often found in the autistic population, including but not limited to exceptional focus, deep interest in certain topics or domains and strong memory. 
%This approach shifts the focus from viewing autism as a condition to be remedied to recognizing it as a natural and valuable form of diversity. 
However, our current study, by focusing solely on the challenges and needs expressed by autistic individuals, intersects with both the neurodiversity and medical models. It attempts to address communication challenges—akin to the medical model—while firmly embracing neurodiversity principles. This includes adopting user autonomy, choice and dynamic feedback rather than rigid directives as a fundamental design choice, and advocating for mutual effort, acknowledging preferences and diversity of communication styles as a natural variation across humans. In the future, we plan to conduct studies specifically with neurotypical users to explore how they can better understand and interact with autistic individuals, and eventually with both user-groups together. This study is the first step in that direction. We elaborate on our vision in \secref{sec:discussion}.
%In this study, we embrace the neurodiversity lens in an attempt to redesign traditional chat applications, tailoring them to better suit the needs of autistic users. 






% To summarize, our study makes these key contributions: 1) We conducted a thorough exploration into how autistic individuals make use of language for self-expression in text-based online conversations, closely examining the nuances of their communication styles. 2) We prototyped a novel chatting interface specifically designed to meet the needs of autistic users. This system was rigorously evaluated in an in-lab setting with six autistic participants, with a focus on its impact on participants' self-expression and comprehension abilities. 3) We gathered detailed feedback on user perceptions of autonomy, accessibility and usefulness of AI-assisted writing, identifying design implications for augmenting existing text-messaging platforms with AI. 










 %While the exact causes of ASD are not fully understood, they are believed to be a complex interplay of genetic and environmental factors, and the management of ASD involves a combination of behavioral therapies, educational support, and sometimes medication. 


==> previous-stuff/introductionPrev.tex <==
\begin{figure}[h]
    \centering
    % First subfigure
    \begin{subfigure}[b]{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/underline-unhovered.png}
        \caption{Ambiguous messages are marked by a grey symbol in the upper left corner of the message box.}
        \label{fig:sub1}
    \end{subfigure}
    \hfill % Spacing between first and second subfigure
    % Second subfigure
    \begin{subfigure}[b]{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/underlined-phrase.png}
        \caption{Hovering the cursor over the message box underlines the ambiguous element. If there are more than 1 ambigous elements, each one is differentiated by a differently colored underline.}
        \label{fig:sub2}
    \end{subfigure}
    \par\bigskip % Spacing between the first row and second row of subfigures

    % Third subfigure
    \begin{subfigure}[b]{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/underlined-explained.png}
        \caption{Clicking on the underlined phrase triggers an explanation to appear.}
        \label{fig:sub3}
    \end{subfigure}
    \hfill % Spacing between third and fourth subfigure
    % Fourth subfigure
    \begin{subfigure}[b]{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/overall-tonemeaning.png}
        \caption{Clicking on any message box causes a description of the message’s tone and meaning to appear.}
        \label{fig:sub4}
    \end{subfigure}
    
    \caption{Demo of {\sc{Interpret}}.}
    \label{fig:interpret}
\end{figure}

\section{Introduction}


% Autism Spectrum Disorder (ASD) is one of the most common neuro-developmental disorder, currently observed at a prevalence rate of approximately 1 in 36 among 8-year-old children in the United States, as per the latest data from the Centers for Disease Control and Prevention (CDC) \cite{cdc-prevalence}. Autistic individuals often experience challenges in communication and social interaction, display restricted interests and repetitive behaviors, and exhibit symptoms that can impair their functional capabilities in educational, occupational, and various other, similar contexts \cite{dsm5}. ASD is referred to as a "spectrum" disorder due to the broad range of symptoms and the varying degrees of severity experienced by autistic individuals. From a medical standpoint, this definition is good.

Autism Spectrum Disorder (ASD) is viewed from a medical lens as a complex neuro-developmental disorder. It is characterized by challenges in verbal and nonverbal communication, difficulties in social interactions, repetitive behaviors, and/or restricted interests \cite{dsm5}. ASD is one of the most common neuro-developmental disorders, currently observed at a prevalence rate of approximately 1 in 36 among 8-year-old children in the United States \cite{cdc-prevalence}. The term `spectrum' in ASD reflects the broad range of symptoms and the varying degrees of severity experienced by autistic individuals. Conversely, the neurodiversity lens, first introduced in the 1990s by autistic sociologist Judy Singer, offers an alternative perspective on autism. Proponents of neurodiversity argue that the challenges encountered by autistic individuals reflect different ways of being that are all part of normal human experiences. 
%They emphasize on the unique strengths often found in the autistic population, including but not limited to exceptional focus, deep interest in certain topics or domains and strong memory. 
This approach shifts the focus from viewing autism as a condition to be remedied to recognizing it as a natural and valuable form of diversity. Our approach intersects the medical and neurodiversity models. It attempts to address communication challenges—akin to the medical model—while firmly embracing neurodiversity principles, emphasizing user autonomy, choice and dynamic feedback rather than rigid directives, acknowledging preferences and diversity of communication styles as a natural variation across humans.
%In this study, we embrace the neurodiversity lens in an attempt to redesign traditional chat applications, tailoring them to better suit the needs of autistic users. 

Prior work in disabilities and linguistics underscores a preference for written communication among autistic individuals, highlighting a tendency towards email and text messaging over FTF interactions \cite{howard-anything-but}. This preference is attributed to the greater control and sensory ease provided by written communication as compared to FTF interactions \cite{nicolaidis-respect-healthcare}. Given the popularity of text-based communication among autistic individuals, it becomes crucial to evaluate whether the design of popular platforms that support text-based communication suffice for their needs. Through focus groups and in-depth qualitative interviews with autistic users, researchers have identified challenges in conveying and interpreting emotional tone and non-literal language, concluding that standard chat features like GIFs and emojis are not sufficient to address these issues. \cite{barros-my-perfect} \cite{page-perceiving-affordances}. Informed by ideation sessions with autistic users and their specific communication needs detailed in these studies, we present a new chatting interface that incorporates three key features not found in traditional chatting applications (\ref{fig:preview-suggest}, \ref{fig:interpret}):
\begin{enumerate}
    \item {\sc Interpret} analyzes the overall tone and meaning of incoming messages, as well as identifies and explains individual potentially ambiguous language elements, such as figurative language, sarcasm, and uncommon emojis.
    \item {\sc Preview} allows users to preview recipients' potential reactions to their messages before sending. It can be activated manually or will automatically engage when a message is detected as blunt, providing feedback on the recipient's potential reaction.
    \item {\sc Suggest} complements {\sc Preview} by generating alternative phrasing for messages deemed blunt. It ensures the original intent of the message is maintained while offering an alternative that is less blunt or not blunt.
\end{enumerate}

Through a rigorous in-lab evaluation with 8 autistic participants, we gathered detailed qualitative feedback and survey responses on participants' a) perceptions of autonomy, accessibility and usefulness of our prototype, and b) use of language for self-expression and interpretation in instant messaging. The results from our 7-point Likert scale survey revealed that 7 out of 8 participants favored continued use of the three main features in their everyday chatting apps, with {\sc{Interpret}} receiving the highest rating (Average 6.25, SD = 1.03), followed by {\sc{Preview}} (Average = 5.88, SD = 1.64), and {\sc{Suggest}} (Average = 5.13, SD = 1.72). Qualitative results showed that our chatting interface enabled convenient clarifications, provided a better alternative to tone indicators, and facilitated constructive reflection on writing technique and style. While our participants demonstrated a strong desire to actively contribute to conversations rather than allowing them to be one-sided, they indicated achieving this balance was challenging in text-based communication. Our work brings to light considerations around the role of user interfaces in appropriating trust levels in AI systems, balancing user autonomy alongside AI-mediation, tradeoffs between real-time intervention and learning in a controlled setting, and the range of users' customization requirements. We believe these considerations have significant implications for the design and deployment of generative AI systems tailored to the specific needs of the autistic community as well as for its broader application.






% To summarize, our study makes these key contributions: 1) We conducted a thorough exploration into how autistic individuals make use of language for self-expression in text-based online conversations, closely examining the nuances of their communication styles. 2) We prototyped a novel chatting interface specifically designed to meet the needs of autistic users. This system was rigorously evaluated in an in-lab setting with six autistic participants, with a focus on its impact on participants' self-expression and comprehension abilities. 3) We gathered detailed feedback on user perceptions of autonomy, accessibility and usefulness of AI-assisted writing, identifying design implications for augmenting existing text-messaging platforms with AI. 










 %While the exact causes of ASD are not fully understood, they are believed to be a complex interplay of genetic and environmental factors, and the management of ASD involves a combination of behavioral therapies, educational support, and sometimes medication. 


==> previous-stuff/limitations.tex <==
\section{Limitations}

There are a number of limitations of our study. Recruiting participants solely from Tufts University restricts the generalizability of our findings to the broader autistic community, due to a lack of diversity in age, background, and education. Additionally, the small sample size of 8 participants further limits the study's scope and the strength of its conclusions. In both phases of our user study, participants engaged with an imaginary character. Participants may have made varying assumptions about their relationship dynamics with Ben, leading to differences in their interactions and responses. While keeping the complexity of this setup minimal, we tried our level best to provide all essential details to participants. Lastly, the in-lab setting of our study may not fully replicate the nuances and dynamics of real-life text messaging, which typically involves more complex and varied stakes.
